VIDAR: Visual-Inertial Dense Alignment and Reconstruction via a Geometric Foundation Model

Monocular foundation models provide dense geometry but usually lack a stable metric scale. This paper presents VIDAR, a visual-inertial dense reconstruction framework that couples SVO+IMU odometry with Depth Anything 3. VIDAR uses the visual-inertial front end as a metric anchor: it provides camera poses, scale, and a consistent world frame for aligning dense foundation-model predictions across time. The foundation model then contributes detailed local geometry that is fused into a global reconstruction. We study both pose-conditioned DA3 and a decoupled alignment strategy. On EuRoC, pose injection reduces scale error to about 1\% and reaches 0.463 mean F@0.10; the decoupled hybrid improves this to 0.676 without ground-truth poses. Results on EuRoC and TUM RGB-D show that VIDAR is a practical route to metric dense monocular reconstruction.

==> sections/06_discussion.tex <==
\section{Discussion}

The experiments support a role-separated design. In visual-inertial EuRoC sequences, SVO+IMU is the most reliable trajectory anchor, while the tested DA3-Streaming poses are not sufficient to replace it. In RGB-only TUM sequences, DA3 is stronger than monocular SVO, showing that learned geometric priors are useful when classical monocular geometry is weak. VIDAR therefore uses SVO+IMU for metric anchoring and DA3 for dense geometry, rather than treating either component as a universal substitute.

The main remaining difficulty is long-sequence fusion. Independently reconstructed DA3 chunks may differ by local deformation, not only by scale, rotation, and translation. A single Sim(3) alignment can therefore be insufficient even if SVO+IMU provides accurate camera poses. This motivates state-carrying reconstruction, DA3-Streaming-style processing, or future pose-conditioned DA3 reconstruction guided by SVO+IMU. The resource sweep reinforces this need: SVO remains below 1~GB peak GPU memory, while DA3 can approach the limit of a 12~GB GPU.

\subsection{Limitations}

Several limitations remain. The TUM DA3 comparisons use tested DA3 settings per sequence, while SVO uses a fixed monocular configuration. Dense-map quality metrics such as completeness, Chamfer distance, and F-score are also not reported. Future work should expand dataset coverage, add point-cloud accuracy metrics, and test a state-carrying or pose-conditioned VIDAR implementation.

